GaDei: On Scale-up Training As A Service For Deep Learning

Deep learning (DL) training-as-a-service (TaaS) is an important emerging industrial workload. The unique challenge of TaaS is that it must satisfy a wide range of customers who have no experience and resources to tune DL hyper-parameters, and meticulous tuning for each user's dataset is prohibitively expensive. Therefore, TaaS hyper-parameters must be fixed with values that are applicable to all users. IBM Watson Natural Language Classifier (NLC) service, the most popular IBM cognitive service used by thousands of enterprise-level clients around the globe, is a typical TaaS service. By evaluating the NLC workloads, we show that only the conservative hyper-parameter setup (e.g., small mini-batch size and small learning rate) can guarantee acceptable model accuracy for a wide range of customers. We further justify theoretically why such a setup guarantees better model convergence in general. Unfortunately, the small mini-batch size causes a high volume of communication traffic in a parameter-server based system. We characterize the high communication bandwidth requirement of TaaS using representative industrial deep learning workloads and demonstrate that none of the state-of-the-art scale-up or scale-out solutions can satisfy such a requirement. We then present GaDei, an optimized shared-memory based scale-up parameter server design. We prove that the designed protocol is deadlock-free and it processes each gradient exactly once. Our implementation is evaluated on both commercial benchmarks and public benchmarks to demonstrate that it significantly outperforms the state-of-the-art parameter-server based implementation while maintaining the required accuracy and our implementation reaches near the best possible runtime performance, constrained only by the hardware limitation. Furthermore, to the best of our knowledge, GaDei is the only scale-up DL system that provides fault-tolerance.

==> compare.tex <==
The two state-of-the-art single node multi-GPU training implementations are mpiT~\cite{mpiT} and DataParallelTable (DPT)~\cite{dpt}, which is based on collective operations provided by nccl\cite{nccl}. mpiT is running on top of MPI~\cite{mpi}, which traditionally does not provide fault-tolerance mechanism, except few research prototypes\cite{mpi-ft}. DPT orchestrates multiple learners in the same process, thus when one learner fails, the entire process is shutdown. Further, nccl implements blocking collective operations, and their behavior in the presence of failure is not defined.

\begin{enumerate}
\item Show NLC workloads that won't converge if using large batch size and high communication frequency, and abysmal speedup number using mpiT.
\item Show a Table that compares PS designs.
\end{enumerate}

\begin{table}[h!]
\centering
\footnotesize{
\begin{tabular}{lcccc}

	                &mpiT  & nickle & CMU-PS   & \Tool \\
Fault-tolerant     	& \No  & \No	& \Yes 	&\Yes\\
High-performance	& \No 	& \No	& \No	&\Yes\\
Formal-method-verfication & \No & \No     & \No	&\Yes\\

\bottomrule
\end{tabular}
}
\wztext{YF: why  mpiT is slow ? , YD: why this is challenging? describe system design stream, threads etc.}
%\nocaptionrule
\caption{A comparison among implementation of PS (\Yes: yes; \No: no). We define high-performance as we can observe speedup on NLC product }
\label{tab:comp}
\end{table}
\wztext{are we going to discuss twitter's torch-ipc ? it doesnt seem to be a mature thing.}
\wztext{Minwei: cloud implication, why single node works well. Long-tail }
\wztext{Li: what kind of workload fits this setup, tightly-coupled system can beat a loosely-coupled system. Can be orthogonal to hierarchical PS. Hardware optimized to the limit. Supporting evidence. when it is most useful}
\wztext{Yandong: scale-up vs scale-out we are scale-up}


==> intro-original.tex <==
\section{Introduction}
\label{sec:intro}


Deep learning (DL) has emerged as an effective approach to many machine learning 
problems, including natural language processing (NLP), image classifications, 
and speech recognition, etc. To deliver high prediction accuracy under limited 
time budget, existing systems~\cite{} commonly resort to parameter server based 
frameworks to scale out the training, leveraging large number of distributed 
CPUs or GPUs to collectively search the model parameters for non-convex deep 
neural network formulations. 


However, with the rapid advancement of GPU devices and corresponding library 
support, such as cuDNN~\cite{}, the communication cost of exchanging models 
between parameter servers and learners over the network is quickly 
diminishing the benefits of scale-out trainings. In addition, many production 
workloads suggest that high accuracy is only achievable with small batch 
sizes, implying the necessity of higher communication frequency to obtain 
high-quality training results. Realizing such an issue, many deep learning 
solution vendors have built specialized scale-up servers to reduce the 
need of network communication without depriving the users of the opportunities 
to leverage multiple GPUs. 
%For example, DevBox introduced by NVIDIA combines 4 Titan X GPUs with 4-way 
%PCI-e3 $\times$ 16 support to specifically serve the deep learning workloads. 


Though the above scale-up servers can efficiently boost the training 
performance, our analysis reveals that the existing iterative model 
synchronization schemes, including mpiT~\cite{} or NCCL~\cite{} used by 
the state-of-the-art deep learning frameworks are still unable to make the 
best use of underlying hardware, due to either the reliance on the 
blocking-based model synchronization or the inability to exploit the 
staleness tolerance. Consequently, the adoption of those mechanisms 
consistently results in GPU stalls, leading to severely degraded device 
utilization ($\le$ 60\%). Furthermore, rigid gradient update methods 
used by the current model synchronization schemes is incapable of 
providing different deep learning models with fast convergence speed.


To conquer those issues, we introduce GaDei, a high-performance 
parameter server, aiming to efficiently coordinate the model 
synchronization among GPUs located on the same machine. In order to 
achieve scalable deep learning for workloads that demand high 
communication frequency, GaDei strives to pipeline the entire model 
synchronization, overlapping all the model training and data movement 
phases to eliminate GPU stalls. Specifically, GaDei synthesizes 
three optimization strategies, including (1) Hogwild-based model 
aggregation to overlap the gradient update with weights pulling, 
(2) on-device double buffering along with multi-streamed design 
to pipeline model trainings and parameter movements, and 
(3) staleness-mitigated batch sizes to guarantee the model 
convergence.  Evaluation with a diverse set of real-world deep 
learning workloads demonstrates that GaDei is able to efficiently 
exploit the bandwidth offered by the commodity scale-up servers, 
providing faster convergence and significantly higher training 
speedups compared to existing open-source solutions, such as mpiT and NCCL. 


Overall, this work has made the following contributions:
\begin{enumerate}
\item We have identified a critical set of deep learning problems 
using real-industry workloads, showing that many deep learning 
services rely on conservatively small batch sizes along with 
high model synchronization frequency to guarantee the convergence, 
so that the training models can serve general public of different datasets.

\item We have designed and implemented a highly-optimized parameter 
server system, called GaDei, to deliver scale-up and resilient 
training for the above workloads on multi-GPU servers. 

\item We have rigorously proved the correctness of the design from 
both training convergence and concurrent programming verification. 
Meanwhile, we have systematically evaluated the performance by 
using 6 different deep learning workloads and compared the 
performance with open-source solutions.
\end{enumerate}

The rest of this paper is organized as follows:
\todo{yandong: continue}


\begin{comment}
\todo{replace jewel and welltok to something else}
\begin{figure*}[t]
\pgfplotstableread[row sep=\\,col sep=&]{\\
  interval & bs1 & bs2 & bs4 & bs8 & bs16 & bs32 & bs64 & bs128 \\
    mr    & 77.6 & 77.2 & 77.6 & 77.2 & 76.7 & 76.7 & 76.6 & 73.9 \\
    age   & 79.8 & 80.5 & 78.0 & 75.9 & 75.1 & 74.6 & 73.7  & 73.0 \\
    yelp  & 62.2 & 63.5 & 62.5 & 63.5 & 61.8 & 62.6 & 62.3 & 62.1  \\
    \welltok  & 63.8  & 60.4 & 54.5 & 44.4 & 24.6 & 6.7 & 0.1 & 0.1\\
    \jewel & 59.7 & 58.4 & 55.4 & 53.7 & 47.5 & 34.6 & 16.8 & 12.8 \\
    }\mydata

\begin{tikzpicture}
    \begin{axis}[
            xbar ,
             y axis line style = { opacity = 0 },
            bar width=.25cm,
            width=\textwidth,
            height=1.1\textwidth,
            legend style={at={(0.5,1.0)},
                anchor=north,legend columns=-1},
            symbolic y coords={mr,age,yelp,\welltok,\jewel},
            ytick=data,
             tickwidth         = 0pt,
    enlarge y limits  = 0.2,
    enlarge x limits  = 0.02,
             axis x line  = none,
            nodes near coords,
            every node near coord/.append style={font=\small},
            nodes near coords align={horizontal},
            xmin=0,xmax=100,
            xlabel={Accuracy in \%},
        ]
         
        \addplot table[y=interval,x=bs1]{\mydata};
         \addplot table[y=interval,x=bs2]{\mydata};
        \addplot table[y=interval,x=bs4]{\mydata};
        \addplot table[y=interval,x=bs8]{\mydata};
        \addplot  table[y=interval,x=bs16]{\mydata};
        \addplot table[y=interval,x=bs32]{\mydata};
        \addplot table[y=interval,x=bs64]{\mydata};
        \addplot table[y=interval,x=bs128]{\mydata};
        \legend{bs1, bs2, bs4, bs8, bs16, bs32, bs64, bs128};
        
    \end{axis}
\end{tikzpicture}
\caption{Accuracy Loss incurred from using large batch size.}
\label{fig:bs}
\end{figure*}
\end{comment}

\section{Background and Motivation}

In this section, we describe a critical set of deep learning problems 
we aim to accelerate on scale-up servers and then we theoretically 
justify the rationale behind the choices of small batch sizes. 

\subsection{Natural Language Processing Workloads}


%Natural language processing (NLP) is one major branch of artificial intelligence (AI). One of the ultimate goal of modern AI is to design a machine which can act humanly and the famous standard to test the intelligence of the machine is the \textbf{Turing Test} proposed by \cite{turingtest}. A machine passes the Turing Test if a human interrogator, after posing some written questions, can not tell whether the written responses come from a person or from a machine \cite{Russell:2009}. To pass the Turing Test, the first capability the machine must acquire is the natural language processing because it must understand human language before going any further.  


%The goal of NLP can be summarized as applying computational models to text or speech data. This paper focuses on the performance optimization perspective for one crucial task of NLP: natural language classification (NLC). The task is to classify input sentence into a category which is one label of a predefined label set. The natural language classification  has been extensively used in many practical applications, e.g. \textbf{(1)} sentiment analysis, the input sentence is classified into label as happy, neutral or angry which represents the sentiment tendency of the writer; \textbf{(2)} topic classification, the input a set of sentences and the output label indicate the topic of the input like news, politics, sports, science etc. ; \textbf{(3)} question classification, for certain application scenario like automatic customer service, all possible answers are predefined into an answer set and represented by a label. So every input question will be classified into a label and corresponding answer will be returned to the customer; \textbf{(4)} author profiling, given input sentences we analyze the gender (the set includes two labels male/female) and age of the author (the label set is the range of human age); \textbf{(5)} evaluation, a label which represents the evaluation according to some standard will be assigned to the input sentence (e.g. assign a score for an English writing exam); \textbf{(6)} intent classification, for certain scenario like dialogue it is required to judge whether the input represents some intention before further processing (the label represents intents like asking time, asking location, requesting weather information, searching for flight information etc.)~. (7) bug detection, the input will be blocks of code or source file and the label represents if the code is bug free or the types of the bug. 


%Current state-of-the-art computational model for sentence classification is based on deep learning \cite{dp,Schmidhuber15,Goodfellow-et-al-2016-Book}. Conventional machine learning techniques mostly process data in their raw form. Hence careful feature design is the crucial factor to the final machine learning system performance. Deep learning focus on automatically capturing discriminating features from the input to make classification or detection. The Convolutional Neural Networks (CNNs) based deep learning model \cite{kalchbrenner-grefenstette-blunsom:2014,kim:2014:EMNLP2014} is the state-of-the-art method for sentence classification. It outperform previous technology like SVM significantly. Figure \ref{fig:nlc_model} demonstrates the CNNs based deep learning model used in this paper.

\begin{figure}[h]
\centering
\smartdiagramset{
uniform color list=NavyBlue!40!white for 7 items,
back arrow disabled=true,
arrow color=black,
uniform arrow color=true,
module y sep=-1,
text width=4cm,
arrow line width=2pt,
module minimum height=0.3cm
}
\smartdiagram[flow diagram]{LookupTable, FullyConnectedLayer(Tanh), Convolution, MaxPooling, FullyConnectedLayer(Tanh), Linear(), Softmax}
\caption{Convolutional Neural Networks (CNNs) based deep learning model.}
\label{fig:nlc_model}
\end{figure}


Although the deep learning brings superior classification accuracy, one known issue is the time consuming training phase. The target of this paper is to boost the training performance of the applications that will be deploy as a service on the cloud, so called "training-as-a-service".  The customers upload their in-house training data to the cloud and the deep networks training will be conducted in the background. The service will be ready for use after the training is finished. Hence from the customer perspective, the turn around time is the model training time. In conclusion, long training time is the pain point for service users. The training time plays a crucial factor in cost and experience for customers and hence minimizing training time has become the top priority task in such kind of applications which is the goal of this paper. 

In order to boost the system performance for neural network training, it is natural to design solutions that utilize multiple computing resources. There are many previous solutions based on server-client framework  and they report good speedup on large scale tasks like CIFAR and ImageNet. However, this type of large scale task does not represent the commercial usage in practices. By examining the real payload data we find the corpus size is less than 10k for most user cases.  We now demonstrate some characters of our tasks.
\textbf{(1) Using large batch size would incur accuracy loss.} Accuracy loss is usually not acceptable for customers. Hence we must boost the training speed without noticeable accuracy loss. We select five representing datasets and demonstrate the accuracy loss with increasing batch size in Figure \ref{fig:bs}. The experiments are conducted on single GPU. The batch size is from 1 to 128. The score to the right side of each horizontal bar is the accuracy. Experimental results prove that using large batch size would result in unacceptable accuracy loss. \textbf{(2) Solution based on distributed training is too expensive.} The bandwidth of cross machine communication is often limited and on the cloud the network can be unstable. Hence designing conventional distributed training framework is too expensive due to the high communication overhead. Current GPU technology advancement is rapid and the computing speed in terms of FLOPS has been increasing every year. On the other hand, NVIDIA's CUDNN library boost the algorithm speed significantly. As a result, there is increasing amount of information to be transferred in unit time and the network bandwidth will be easily saturated. One way of handle this communication bottleneck is to turn on the staleness mode which will set local worker do more work (more mini batches) before it synchronize with the server. However, increasing staleness would often result in accuracy loss. The last two rows of Table \ref{tab:mpiT_staleness_compare} show that if the worker always communicate with the server after it finishes each mini batch (no staleness), then only less 10 percent of time is utilized for real calculations and the majority time (>90\%) is used for communication.  In the Table \ref{tab:mpiT_staleness_compare},  efficiency 7.9 means for the worker only 7.9 percent of time is used for calculations. If  the staleness is increased to 8, the efficiency is boosted significantly. However, there is also significant accuracy loss. Even when there is no staleness,  accuracy loss appears in several tasks (especially yelp and age). \textbf{(3) Little or zero hyper parameter tuning opportunity is feasible.} The performance of distributed training, including both accuracy and communication overhead, is hyper parameter sensitive. For application scenario like cognitive service on the cloud, users have neither expertise nor time for hyper parameter tuning. The ease of use is a crucial design consideration. Compared to the routines of large amount of tuning experiments in R\&D environment, customers just upload the training data and then expect a well trained model to be ready in short period to use. As a result, the hyper parameters will be preset to be fixed values (or a set of fixed values for different scenarios) and in order to cover diverse use cases, hyper parameters will be set in highly conservative way (small mini batch size and small learning rate). 



\begin{table*}[htbp]
\centering
\begin{tabular}{|l|r|r|r|r|r|}
\hline
 &  \textbf{\jewel} & \textbf{\welltok} & \textbf{yelp} & \textbf{age} & \textbf{mr} \\ \hline
\textbf{Single GPU Accuracy} & 58.4 & 60.4  & 62.6 & 81.0 & 77.2 \\ \hline
\textbf{12 GPU Workers Accuracy (no staleness)} & 57.7 & 57.8  & 56.9 & 74.1 & 77.2 \\ \hline
\textbf{12 GPU Workers Accuracy (staleness=8)} & 39.8 & 55.1  & 20.0 & 63.6 & 50.0 \\ \hline
\textbf{12 GPU Workers Efficiency (no staleness)} & 7.9 & 4.9 & 8.8 & 4.0 & 5.5  \\ \hline
\textbf{12 GPU Workers Efficiency (staleness=8)} & 35.8 & 29.4 & 42.9 & 24.9 & 33.7  \\ \hline
\end{tabular}
\caption{Accuracy loss with staleness under distributed training framework. The unit of this table is percentage. Efficiency 7.9\% represents   for the worker only 7.9 percent of time has been used for real calculations, the rest part of time (92.1\%) is used for communication.}
\label{tab:mpiT_staleness_compare}
\end{table*}



In summary, we elaborate on the motivation of this work in this subsection. \textbf{(1)} We introduce the natural language classification task and give examples to show that this task has been widely used in practice.
\textbf{(2)} We then explain why it is important to improve the training performance as the application is deployed as service on the cloud and reduce training time equals less cost and better experiences for customers.
\textbf{(3)} Many previous work present solutions that are suitable for large scale computer vision tasks like CIFAR and ImageNet, we argue that type of solution does not represent the commercial applications in practices. There lacks of researches for commercial applications that this work focuses on.
\textbf{(4)} We describe some characters of the workload that we want to optimize. Solid evidence have been presented to show that previous main stream method like client-server based framework is not suitable for our tasks and finally we demonstrate the need of having a dedicated design for this kind of application.    


\subsection{Compare to other frameworks}
\input{compare}

\subsection{Why small batch size is appropriate for asynchronous parallelism?}
\label{sec:smallbs_justification}
\input{batchsize}

%\subsection{Contribution}
%\begin{enumerate}
%\item Identify an important problem using real industry workload: small batch size, high communication frequency
%\item Design and implement a highly-optimized system that outperforms opensource ones and for the first time shows that it can achieve speedup on such workload on commodity systems
%\item Proves the correctness of such system and provides fault-tolerance
%\item Make suggestions to hardware designers as what kind of memory throughput we need for modern DL systems.
%\end{enumerate}


==> optim.tex <==
\section{System Optimization}
\label{sec:optim}
\subsection{What works}
\begin{enumerate}
\item fine-granularity locking
\item staging GPU memory as a buffer to enable async copy
\item lock-free on weights
\item NUMA-aware? but how do we do it and how to show result ?
\item SSE ? 
\end{enumerate}

\subsection{What could have worked but don't, and why}
\begin{enumerate}
\item 16 bit representation, s/w conversion too slow; and all kinds of compression work (unless it can be done efficiently on GPU
\item lock-free. too much spins on client

\end{enumerate}



==> outline.tex <==
\section{Outline and Plan}
\subsection{Outline}
\begin{enumerate}
\item Motivation. Why it is important (in general DL is important, and in particular NLC is important, we evision DL as a servce, also look at Cloud view paper from Berkeley, to see why they dont like xxx as a service term ? How representative the workload is ? Why the enterprise client workload is important. Show the plots with large batch size things are not converging, explain the label number is large, a very difficult task. Also, why batch size is small -- we need a model that is uniformally applicable to all the customers. Need to strike that one communication hop out of a computer puts accuracy under the water (in connection with hogwild! even lost the accuracy here), maybe we can use Nexus to do the experiments -- the implication for cloud then is bad. But can we also have a large dataset, like YELP (but possibly with more labels), to back this up ? And why we need to run up to 200 epochs ( for the product purpose, to be really safe that we need to run long). Motivation: we want really fast training -- grand goal, people slide the mouse and the accuracy is out. 
\item Design and implementation. (1) Queue abstraction, coarse granualarity, fine granularity, , PS on GPU(probably not, need to argue that memcpy to GPU is not worth it) (2) we stick to ASGD  (3) We are going to do fault-tolerant. (4) We are going to do LuaRocks. that it can support any SGD based algorithm -- Logistic regression, RNN and etc (5) Why we didnt use two condition variables for fine-granualarity locking -- b/c we need PS not to wait, but Worker to yield (5) Question: will TLB huge table help ? I seem didnt get it to work (6) Can we just argue why lock-free wouldn't outperform ? (7) socket-aware, especially on softlayer k80 machines ? (8) SSE
\item System modeling. (1) Training, communication, use benchmark measurement (e.g., our prevous feasibility study) to argue why bandwidth is such a key and why other approach (even involve just one extra memcpy will not work ? ) (2) can we get something that if PS update takes a bit longer, what the overall effect is. What is the critical path, and etc.  what about the effect of parameters update timing. Can we deduce what is the critical path by measuring each component. (3) are we going to model hyper-threading effect ? (note on K80 we can even run faster than digits, because we have more  CPU cores and we turned off the hyper-threading there) (4) are we gonna model-testing, since it also takes CPU or GPU resources? 
\item Fault-tolerance modeling. Not to bring dead learner back (e.g., not elastic) How do we inject failure (randomly kill stuff ? )
\item Methodology (1) h/w K80 (maybe digits) (2) Benchmark explanation. (2.1) private dataset (NLC): word-embedding, different layer structure? (2.2) imagenet/cifar dataset, alexnet, VGG, GoogleNet ?  
\item Evaluation (1) Only show fast kernel (show GPU utility), speedup on PCI-e 3rd generation (2) vs mpiT, vs nickle, (CMU-PS?, can we just use micro-benchmark ) (3) compare with different queue implementation (e.g. coarse granularity locking)  (4) we shall show for each optimization, what kind of gain we get, my guess is that finer granualrity locking and lock-free parameter update are the most important.
\item Misc rebuttal that hogwild! would not work, if we are not careful about sending gradients, maybe also argue why that is why relying on any highlevel MPI will not be enough (i.e., probably similar to why use stream wait is not gonna be not sufficient). However, we should mention that w.r.t parameters, we can use lock free, we can even show that w/ lock and w/o lock performance, and we shall show for each optimization, what kind of gain we get, my guess is that finer granualrity locking and lock-free parameter update are the most important. 
\item Program Correctness argument: (1) (i) why no-deadlock (consider all possible waiting scenario, and model possibly via SMT solver (Yunhui), to query that there is no deadlock. (ii) data-race , gradients cannot tolerate data race (rebut the hogwild! paper, need help from Liu Ji, but weights can (using IJCAI staleness argument)
(2) why fault tolerance model is correct: (i) why 1 learner eventually can get to the correct result eventually -- simple math argument (Liu Ji) (ii) why terminate  ?
Failure detection mechanism: nanny process (consider this process really robust, and ping others to detect if they are still alive)  
\item (1) Future compute arch design: memory bandwidth, nv link, do we show how PCI-e speed grow with GPU speed (we can also show that nvidia-smi GPU utility, and show tradeoff among fast/slow kernel, fast/slow PCI-e) does it grow fast enough (question: is it gonna be a general enough statement, is this universally true for other type of workload ? cite Sina's sigmod paper ?). (2) Can we predict until when we see no speedup anymore.  
\item Related works: (1) Motivation-wise: compare to imagnet, i.e., specific type of workload. do people use AlexNet for all kinds of workload, or just use it as a feature extractor, cite rudra and Ji's papers to make the argument that more updates mean better convergence. (2) Performance-wise: mpiT, nickle, ?CMU-PS? (write a big table , that compares performance, and if supports fault-tolerant, maybe goes to intro. (3) fault-tolerant: CMU-PS and what else ? (4) use IPC , cite Grace (oopsla'09) ; use posix based tool, cite Weiwei's paper for correctness argument. (4) cite ICT's papers to argue memory bandwidth is an issue  
\item Future work: model averaging ? Is there any benefit to do distributed training, if there are 16 GPUs on the same node -- a tightly coupled system is more controllable in a cloud enviroment.
\end{enumerate}

\subsection{Plan}


==> overview.tex <==
\section{Background and System Modeling}
\label{sec:overview}
In this section, we first introduce the background of deep learning solving algorithm, in particular Stochastic-SGD (SGD) and define the terminologies we use in this paper. We then describe the performance modeling of our parameter server design and the required memory bandwidth to achieve speedup. 

\subsection{Terminology Definition}
In essence, deep learning problem solves the following generic optimization problem \[ \min_\theta \quad F (\theta) \assign \frac{1}{N} \sum_{n = 1}^N f_n(\theta), \] where $\theta$ is the parameter vector we are pursuing,
$N$ is the number of samples, and $f_i(\theta)$\footnote{$f(\theta)$ is typically a multi-layered neural network with differentiable activation function.} is the loss function
for the $i^{\text{th}}$ sample.


The underlying algorithm used in deep learning is SGD (stochastic gradient descent). SGD iterates overall the entire training dataset, and apply Equation~\ref{eqn:gd} for each training sample. In Equation~\ref{eqn:gd}, $i$ is the iteration number, $k$ is the k-th parameter, $\alpha$ is the learning rate, $\nabla$ is the differential operator. SGD passes through the entire training dataset several times until the model converges. Each pass is called Epoch(denoted by $E$). To improve computation efficiency, one can group a number of samples (mini-batch) and still apply Equation~\ref{eqn:gd} to update weights, where $i$ denotes the $i$-th minibatch.
\begin{equation}
  \theta^{(k)}(i+1) = \theta^{(k)}(i) - \alpha\nabla \theta^{(k)}(i) \label{eqn:gd}
\end{equation}


To accelerate deep learning training, practitioners usually adopt the Parameter Server architecture. Figure~\ref{fig:design_base} illustrates a typical parameter server architecture. Each \textit{learner} retrieves a mini-batch of training samples from storage , calculates gradients and send the gradients to the parameter server. Parameter Server then updates its weights by applying gradients update rules. Before calculating the next gradients, \textit{Learner} pulls weights from the parameter server. In this paper, we use $\lambda$ to represent number of learners. Two most-widely adopted parameter server communication protocols are synchronous SGD (SSGD) and Asynchronous SGD (ASGD). Equation~\ref{eqn:ssgd} describes the weight update rule used in SSGD. Parameter server collects gradient from each learner and the weights update rule is defined in Equation~\ref{eqn:ssgd}. SSGD is mathematically equivalent to SGD, when $\lambda \times \mu$ is equal to the batch size used in SGD.    
\begin{equation}
	\begin{aligned}
		\nabla \theta^{(k)}(i) &= \frac{1}{\lambda}{\sum_{l=1}^{\lambda} \nabla\theta_{l}^{(k)}}\\
		\theta^{(k)}(i+1) &= \theta^{(k)}(i) - \alpha\nabla \theta^{(k)}(i)
	\end{aligned}
 \label{eqn:ssgd}
\end{equation}

SSGD is not computation efficient because the parameter server keeps learners from executing until it collects gradients from all the learners and update the weights. ASGD relaxed such constraints by applying gradient update rule , which is defined in Equation~\ref{eqn:asgd}, whenever a gradient is sent by any learner. While ASGD has the obvious runtime performance advantage over SSGD, it inevitably introduces staleness in the system and it may slow down convergence speed. As discussed in Section~\ref{sec:smallbs_justification}, using small mini-batch size can counter staleness in the system, several works~\cite{mpiT,liu-asgd-nips-2015, zhang-ijcai-2016} also demonstrate there exist techniques that can achieve similar model accuracy (typically $\pm 1\%$), using dozens of learners, in the ASGD setup compared to SSGD when fixing the training epochs. When measuring ASGD speedup, $T_{1}$ is the time for a single learner SGD algorithm to train $E$ epochs. $T_{2}$ is the time for ASGD algorithm to train $E$ epochs. Speed up is defined as $\frac{T1}{T2}$. To ensure a fair comparison, one must certify the model accuracy trained by ASGD is similar to that of SGD.

\begin{equation}
\begin{aligned}
\Delta \theta^{(k)}(i) &= \Delta\theta_{l}^{(k)}, L_{l} \in {L_{1}, ..., L_{\lambda}} \\
\theta^{(k)}(i+1) &= \theta^{(k)}(i) - \alpha\Delta \theta^{(k)}(i)
\end{aligned} 
\label{eqn:asgd}
\end{equation}

\begin{figure}
\begin{center}
%\centering
\includegraphics[scale=0.5]{./figures/design_base-crop}
\caption{A typical parameter server architecture.}
\label{fig:design_base}
%\vspace{-1cm}
\end{center}
\end{figure}




\subsection{System Modeling}
\label{sec:modeling}
Each learner has three time components: $T_{train}$, $T_{pull}$, $T_{push}$. Assume $T_{apply}$ is the time where PS grabs a gradient and updates the weight once. 
In SSGD,  to achieve any speedup, we must have $T_{train} \ge (T_{push} + T_{pull} + T{apply})$. In ASGD,  push and pull operations may overlap, to achieve any speedup, we must have $T_{train} \ge (T_{push} + T{apply})$ (apply update and push cannot overlap, since apply update can only start when gradients are pushed to the parameter server side). Note that the operation conducted on the PS side is always level 1 BLAS operation, thus it is entirely bounded by the memory throughput. Since combined memory bandwidth between GPU and CPU and memory bandwidth used in CPU DRAM are of the same order of magnitude. We can infer the required memory bandwidth to observe any speedup is at least $\frac{2 \times ModelSize}{TrainTime_{per minibatch}}$  Table~\ref{tab:bandwidth_requirement} records the minimal bandwidth requirement to observe any speedup. To see $X$ speedup, we need to multiply that requirement by a factor of $X$. As we can see, the requirement for commercial workload is quite high.

\begin{table*}[htbp]

\begin{tabular}{|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\hline
\multicolumn{ 1}{|l|}{} & \multicolumn{ 2}{l|}{\textbf{jewel}} & \multicolumn{ 2}{c|}{\textbf{\welltok}} & \multicolumn{ 2}{c|}{\textbf{Age}} & \multicolumn{ 2}{c|}{\textbf{Yelp}} & \multicolumn{ 2}{c|}{\textbf{CIFAR }} & \multicolumn{ 2}{c|}{\textbf{ImageNet}} \\ \cline{ 2- 13}
\multicolumn{ 1}{|l|}{} & \multicolumn{ 2}{l|}{\textbf{2.46K,7.69MB}} & \multicolumn{ 2}{c|}{\textbf{500K,98.60MB}} & \multicolumn{ 2}{c|}{\textbf{68.48K,72.86MB}} & \multicolumn{ 2}{c|}{\textbf{500K,98.60MB}} & \multicolumn{ 2}{c|}{\textbf{50K,59,97MB}} & \multicolumn{ 2}{c|}{\textbf{1280K,244.48MB}} \\ \cline{ 2- 13}
\multicolumn{ 1}{|l|}{\textbf{$\mu$}} & \multicolumn{1}{l|}{\textbf{TPE}} & \multicolumn{1}{l|}{\textbf{RB}} & \multicolumn{1}{l|}{\textbf{TPE}} & \multicolumn{1}{l|}{\textbf{RB}} & \multicolumn{1}{l|}{\textbf{TPE}} & \multicolumn{1}{l|}{\textbf{RB}} & \multicolumn{1}{l|}{\textbf{TPE}} & \multicolumn{1}{l|}{\textbf{RB}} & \multicolumn{1}{l|}{\textbf{TPE}} & \multicolumn{1}{l|}{\textbf{RB}} & \multicolumn{1}{l|}{\textbf{TPE}} & \multicolumn{1}{l|}{\textbf{RB}} \\ \cline{ 2- 13}
\multicolumn{ 1}{|l|}{} & \multicolumn{1}{l|}{\textbf{(sec)}} & \multicolumn{1}{l|}{\textbf{(GB/s)}} & \multicolumn{1}{l|}{\textbf{(sec)}} & \multicolumn{1}{l|}{\textbf{(GB/s)}} & \multicolumn{1}{l|}{\textbf{(sec)}} & \multicolumn{1}{l|}{\textbf{(GB/s)}} & \multicolumn{1}{l|}{\textbf{(sec)}} & \multicolumn{1}{l|}{\textbf{(GB/s)}} & \multicolumn{1}{l|}{\textbf{(sec)}} & \multicolumn{1}{l|}{\textbf{(GB/s)}} & \multicolumn{1}{l|}{\textbf{(sec)}} & \multicolumn{1}{l|}{\textbf{(GB/s)}} \\ \hline
1 & 5.61 & 7.00 & 25.22 & 11.50 & 574.80 & 17.36 & 4376.12 & 22.53 & \multicolumn{1}{l|}{N/A*} & \multicolumn{1}{l|}{N/A*} & \multicolumn{1}{l|}{N/A*} & \multicolumn{1}{l|}{N/A*} \\ \hline
2 & 3.22 & 6.10 & 14.11 & 10.28 & 309.51 & 16.12 & 2367.04 & 20.83 & 792.45 & 3.78 & 26957.54 & 11.61 \\ \hline
4 & 1.77 & 5.54 & 7.46 & 9.72 & 169.99 & 14.68 & 1299.42 & 18.97 & 502.63 & 2.98 & 15596.41 & 10.03 \\ \hline
8 & 1.00 & 4.89 & 4.06 & 8.93 & 104.39 & 11.95 & 802.04 & 15.37 & 356.46 & 2.10 & 9499.38 & 8.24 \\ \hline
16 & 0.75 & 3.27 & 2.79 & 6.49 & 77.79 & 8.02 & 571.10 & 10.79 & 290.95 & 1.29 & 7294.30 & 5.36 \\ \hline
32 & 0.72 & 1.69 & 2.38 & 3.82 & 69.52 & 4.49 & 451.61 & 6.82 & 261.23 & 0.72 & 5769.76 & 3.39 \\ \hline
64 & 0.80 & 0.76 & 2.37 & 1.91 & 77.14 & 2.02 & 403.69 & 3.82 & 245.68 & 0.38 & 5014.85 & 1.95 \\ \hline
128 & 1.00 & 0.31 & 2.77 & 0.82 & 100.22 & 0.78 & 402.97 & 1.91 & 234.38 & 0.20 & 4784.22 & 1.02 \\ \hline
\end{tabular}
\caption{Minimum bandwidth requirement to see any speedup. $\mu$ is mini-batch size, TPE stands for Time Per Epoch, RB stands for Required Bandwidth. *Both CIFAR and ImageNet use models that use Batch Normalization (BN), which requires $\mu \geq 2$.}
\label{tab:bandwidth_requirement}
\end{table*}






